Joint Effects of Context and User History for Predicting Online Conversation Re-entries

As the online world continues its exponential growth, interpersonal communication has come to play an increasingly central role in opinion formation and change. In order to help users better engage with each other online, we study a challenging problem of re-entry prediction foreseeing whether a user will come back to a conversation they once participated in. We hypothesize that both the context of the ongoing conversations and the users' previous chatting history will affect their continued interests in future engagement. Specifically, we propose a neural framework with three main layers, each modeling context, user history, and interactions between them, to explore how the conversation context and user chatting history jointly result in their re-entry behavior. We experiment with two large-scale datasets collected from Twitter and Reddit. Results show that our proposed framework with bi-attention achieves an F1 score of 61.1 on Twitter conversations, outperforming the state-of-the-art methods from previous work.

==> ACL2019(final)/figs/case_attention.tex <==
\begin{figure}[t]
\setlength{\belowcaptionskip}{-3mm}
\begin{center}
\includegraphics[width=0.4\textwidth]{figs/attention.pdf}
%\vskip -0.5em
\captionsetup{font=10pt}
\caption{
%\lu{updated}
Attention output of model \textsc{BiLSTM+BiA} for the two sample conversations in Figure~\ref{fig:intro-example}. 
%It assigns higher weights to conversation 2 by aligning it to $\bf {U_1}$'s chatting history. A higher re-entry probability is then predicted for conversation 2. 
}\label{fig:attention}
%\vskip -1em
\end{center}
\end{figure}

==> ACL2019(final)/figs/framework.tex <==
\begin{figure}[t]
\includegraphics[width=75mm]{figs/model.pdf}
%\vskip -0.5em
\captionsetup{font=10pt}
\caption{
%\lu{explain notations on c, C, T, h, H, D; the fig takes too much space, and need to make the words sharper}
The generic framework for re-entry prediction. We implement it with three encoders (Average Embedding, CNN, and BiLSTM) for turn modeling and four mechanisms (Simple Concatenation, Attention, Memory Networks, and Bi-attention) for modeling interactions between context and user history.
% $u$: the target user. $c$: the target conversation.
% $t_i,a_i$: the words and auxiliary information of a turn in $c$'s context. 
% $m_j$: a message in $u$'s chatting history. 
% $H^T$: turn modeling outputs. $H^U$: user history modeling outputs. 
% ${\bf r}^O$: the representations produced by interaction layer. $p(u,c)$: the final prediction.
}
%\vskip -1em
%\vspace{-1em}
%\xingshan{Looks like a little too long for caption. I am not sure whether we need to explain the notations again here, since we have explained them in main body.}
\label{fig:mod}
\end{figure}

==> ACL2019(final)/figs/intro-example.tex <==
% \begin{figure}\small
%     \centering
%         \begin{tabular}{|p{7cm}|}
%             \hline \underline{\textbf{The user history of $\bf U_1$:}}\\
%           H$_1$: Is there literally no one on twitter who wants to talk about LET ME IN with me? :(\\
%           H$_2$: I think the change in overall tone was enough to let LMI stand on it's own. Love Giacchino's score too.\\
%           H$_3$: I think if i had seen LMI again before making my top ten it would have made the cut. Oh well.\\
%           H$_4$: it's not as bad as I remembered on the blu-ray. Looks like shit next to Avatar, but so does everything lol\\
%           ...\\
%           \hline
%           \hline
%           \underline{\textbf{ Conversation 1:}}\\
%           T$_1[$U$_2]$: Instead of focusing on when Oscars got it wrong... Let's talk about when the Oscars got it right...\\
%           \textcolor{blue}{T$_2[\bf{U_1}]$: \textit{The Hurt Locker, The Departed, NCFOM, LOTR, Schindler's List, Braveheart, Gladiator, The Godfather Part 1 \& 2}}\\
%           ...\\
%           \hline
%           \hline
%             \underline{\textbf{ Conversation 2:}}\\
%             ...\\
%           T$_1[$U$_3]$: Almost fell asleep in the first hour of INCEPTION. In the theatre.\\
%           T$_2[$U$_4]$: lol do you not like it?\\
%           T$_3[$U$_5]$: Meh. MEMENTO $=$ far better film.\\
%           \textcolor{blue}{T$_4[\bf {U_1}]$:\textit{ apples and oranges, plain and simple}}\\
%           ...\\
%           ------------------------------------\\
%           \textcolor{blue}{T$_5[\bf {U_1}]$: \textit{Inception and Memento. Same filmmaker, but completely different scope, themes, ideas, genres, etc.}}\\
%             \hline
%         \end{tabular}
%         \vskip -0.5em
%     \caption{
%     %\lu{it might be better to use some color, in addition to the boldface, easier for readers to see the re-entry}
%     \jing{U1's turns in blue.}
%     Sample tweets in the user history of $\bf U_1$ and two Twitter conversation snippets $\bf U_1$ once engaged in. H$_i$: the $i$-th tweet in $\bf{U_1}$'s history. T$_i[$U$_j]$: the $i$-th turn posted by U$_j$. The blue and italic turns are posted by $\bf U_1$. $\bf U_1$ didn't comes back to Conversation 1 but return to Conversation 2. }
%     \vskip -1em
%     \label{fig:intro-example}
% \end{figure}
\begin{figure}
\hspace{-2mm}
\includegraphics[width=80mm]{figs/example.pdf}
%\vskip -0.5em
\captionsetup{font=10pt}
\caption{
%\lu{remove "the" in "the user history of u1", the arrows are busy, I think we can just highlight the movie names}
Sample tweets in the chatting history of user $\bf U_1$ and two Twitter conversation snippets $\bf U_1$ engaged in.  $\bf H_i$: the $i$-th tweet in $\bf{U_1}$'s history. 
$\bf T_i$[$\bf U_j$]: the $i$-th turn posted by $\bf U_j$. 
First entries by $\bf U_1$ are highlighted in blue in both conversations. $\bf U_1$ only returns to the second one.
% The blue turns are the first entry of $\bf U_1$. The red turn is the re-entry of $\bf U_1$. $\bf U_1$ doesn't come back to Conversation 1 but returns to Conversation 2.
}
\vskip -1em 
\label{fig:intro-example}
\end{figure}

==> ACL2019(final)/figs/statistics_distribution.tex <==
\begin{figure}[t]
\centering
\subfigure[User history]{
\includegraphics[width=0.22\textwidth]{figs/distribution_his_len.pdf}\label{subfig:user-history}
}
\subfigure[Conversation context]{
\includegraphics[width=0.225\textwidth]{figs/distribution_turn_num.pdf}\label{subfig:conv-context}
}
%\vskip -1em
\captionsetup{font=10pt}
\caption{
Distributions of message number in user history and turn number in conversation context on the two datasets. 
%Data distributions on user history and conversation context on our two datasets. 
}
%\vskip -1em
\label{fig:distribution}
\end{figure}

==> ACL2019(final)/figs/varying_context.tex <==
\begin{figure}[t]
\centering
\subfigure[Twitter Dataset]{
\includegraphics[width=0.223\textwidth]{figs/diff_times_twitter.pdf}
}
\subfigure[Reddit Dataset]{
\includegraphics[width=0.22\textwidth]{figs/diff_times_reddit.pdf}
}
%\vskip -1em
\captionsetup{font=10pt}
\caption{
%\lu{x-axis: \# of posts/messages (use the word in the paper, i saw messages are also used) by the user in a given conversation; then you can explain more in the caption}
%\xingshan{Not sure is it clearer?}
%F1 score results for models when given different lengths of context in target conversation. 
F1 scores for prediction on the first, second, and third re-entries (given the conversation context until the last entry). 
%$x$-axis: \# of turns from target user observed in context. %$y$-axis: F1 scores.
%The numbers in x-axis mean the number of messages that the user has posted (i.e. entry times) in given conversation context. 
%For each type of re-entry prediction, 
X-axis: \# of turns in the given conversation context.
Both figures, from left to right, show the F1 scores by \textsc{All-Yes}, \textsc{CCCT}, \textsc{BiLSTM}, \textsc{BiLSTM+MEM}, and \textsc{BiLSTM+BiA}. 
%Our model yields consistently better performance than all comparisons.
%In general, given more entry times, predicting performance gets better for all models.
}
%\vskip -1.0em
\label{fig:diff_times}
\end{figure}

==> ACL2019(final)/figs/varying_history.tex <==
\begin{figure}[t]
\setlength{\belowcaptionskip}{-4mm}
\centering
\includegraphics[width=0.40\textwidth]{figs/diff_length.pdf}
%\vskip -0.5em
\captionsetup{font=10pt}
\caption{ 
%\lu{is this first re-entry prediction or for all re-entry prediction?}
F1 scores of model \textsc{BiLSTM+BiA} on first re-entry prediction, with varying numbers of chatting messages given in user history. 
%F1 score results for our model towards users that have different numbers of history messages. 
%\lu{how the length is measured? you mean tot number of posts in the conversation thus far?}
}
%\vskip -1em
\label{fig:diff_len}
\end{figure}

==> ACL2019(final)/sections/conclusion.tex <==
\section{Conclusion}

%We present a novel neural framework for re-entry prediction, via jointly encoding conversation context and user chatting history. 
We study the joint effects of conversation context and user chatting history for re-entry prediction. 
A novel neural framework is proposed for learning the interactions between two source of information.
Experimental results on two large-scale datasets from Twitter and Reddit show that our model with bi-attention yields better performance than the previous state of the art. 
Further discussions show that the model learns meaningful representations from conversation context and user history and hence exhibits consistent better performance given varying lengths of context or history. 
We also conduct a human study on the first re-entry prediction task. 
%humans and our model is also presented, suggesting that the re-entry prediction task is essentially challenging. 
Our proposed model is observed to outperform humans, benefiting from its effective learning from large-scaled data.

==> ACL2019(final)/sections/experiment.tex <==
\section{Experimental Setup}
\label{sec:expsetup}
\paragraph{Data Collection and Statistic Analysis.} 
To study re-entry behavior in online conversations, we collected two datasets: one is released by \citet{DBLP:conf/naacl/ZengLWBSW18} containing Twitter conversations formed by tweets from the TREC 2011 microblog track data\footnote{\url{https://trec.nist.gov/data/tweets/}} (henceforth \textbf{Twitter}), and the other is \textit{newly collected} from Reddit (henceforth \textbf{Reddit}), a popular online forum. In our datasets, the conversations from Twitter concern diverse topics, while those from Reddit focus on the political issues. Both datasets are in English.

%In the following, we describe how we build the Reddit dataset. 
To build the Reddit dataset, we first downloaded a large corpus publicly available on Reddit platform.\footnote{\url{https://www.reddit.com/r/datasets/comments/3bxlg7/i_have_every_publicly_ available_reddit_comment/}} Then, we selected posts and comments in subreddit ``politics'' posted from Jan to Dec 2008. Next, we formed Reddit posts and comments into conversations with replying relations revealed by the ``\textit{parent\_id}'' of each comment. Last, we removed conversations with only one turn.

In our main experiment, we focus on {\it first re-entry} prediction, i.e. we predict whether a user $u$ will come back to a conversation $c$, given current turns until $u$'s first entry in $c$ as context and $u$'s past chatting messages (posted before $u$ engaging in $c$). 
%(all the messages that posted before the first entry based on the posting time). 
%\xingshan{add some details for data spliting.}
%\jing{Updated the wordings.}
For model training and evaluation, we randomly select $80$\%, $10$\%, and $10$\% conversations to form training, development, and test sets.
%ensuring training conversations are not used in validation and test.  \lu{why saying ensuring, it will not right? unless you divide conversations?} 

%As can be seen, users who engages in a conversation less than twice on average are more likely to abandon a discussion. %instead of coming back. 

\input{tables/statistics.tex}

The statistics of the two datasets are shown in Table \ref{tab:stat}. As can be seen, users participate twice on average in Twitter conversations, and the number is only $1.3$ on Reddit. This results in the severe imbalance over instances of re-entry and non re-entry (negative samples where users do not come back) on both datasets. Therefore, strategies should be adopted for alleviating the data imbalance issue, as done in Eq. (\ref{loss}). 
%\lu{again need to say values to show how to handle the imbalance}
It indicates the sparse user activity in conversations, where most users engage in a conversation only once or twice.
Thus predicting user re-entries only with context will not perform well, and the complementary information underlying user history should be leveraged.



We further study the distributions of message number in user history and turn number in conversation context on both datasets. 
As shown in Figure \ref{fig:distribution}, 
%the distributions in general follow power law.
there exists severe sparsity in either user history or conversation context.
Thus combining them both might help alleviate the sparsity in one information source.
We also notice that Twitter and Reddit users exhibit different conversation behaviors. Reddit users tend to engage in more conversations, resulting in more messages in user history (as shown in Figure \ref{subfig:user-history}). Twitter users are more likely to stay within each conversation, leading to lengthy discussions and larger re-entry frequencies on average, as shown in Figure \ref{subfig:conv-context} and Table \ref{tab:stat}.

\input{figs/statistics_distribution.tex}

\paragraph{Data Preprocessing and Model Setting.}

For preprocessing Twitter data, we applied Glove tweet preprocessing toolkit~\cite{pennington2014glove}.\footnote{\url{https://nlp.stanford.edu/projects/glove/preprocess-twitter.rb}}
For the Reddit dataset, we first applied the open source natural language toolkit (NLTK)~\cite{loper2002nltk} for word tokenization.
Then, we replaced links with the generic tag ``URL'' and removed all the non-alphabetic tokens. 
For both datasets, a vocabulary was built and maintained in experiments with all the tokens (including emoticons and punctuation) from training data.

For model setups, we initialize the embedding layer with $200$-dimensional Glove embedding~\cite{pennington2014glove}, where Twitter version is used for our Twitter dataset and the Common Crawl version applied on Reddit dataset.\footnote{\url{https://nlp.stanford.edu/projects/glove/}}
All the hyper-parameters are tuned on the development set by grid search.
The batch size is set to $32$.
Adam optimizer \cite{kingma2014adam} is adopted for parameter learning with initial learning rate selected among $\{10^{-3},10^{-4},10^{-5}\}$. 
For the BiLSTM encoders, we set the size of their hidden states to $200$ ($100$ for each direction).
For the CNN encoders, we use filter windows of $2$, $3$, and $4$, each with $50$ feature maps.
In MemN2N interaction mechanism, we set hop numbers to $3$.
In the learning loss, we set $\mu=1$ and $\lambda=2$, the weights to tackle data imbalance.
%\lu{you say here! maybe mention earlier}
For re-entry prediction, a user is considered to come back if the estimated probability for re-entry is larger than $0.5$.

\paragraph{Baselines and Comparisons.} 
For comparisons, we consider three baselines. 
\textsc{Random} baseline: randomly pick up a ``yes-or-no'' answer.
\textsc{History} baseline: predict based on users' history re-entry rate before current conversation, which will answer ``yes'' if the rate exceeds a pre-defined threshold (set on development data), and ``no'' otherwise. 
(For users who lack such information before current conversation, it predicts ``yes or no'' randomly.)
%history conversations, which means that if the user tends to re-enter conversations previously, we will answer ``yes'', otherwise ``no'' (if the user doesn't have any history conversations, it will be a random prediction).
\textsc{All-Yes} baseline: always answers ``yes'' in re-entry prediction. 
%This baseline comes from the idea that 
Its assumption is that users tend to be drawn back to the conversations they once participated by the platform's auto messages inviting them to return.
%\jing{Updated the wordings.}
%receive a notification if someone replies to them (both on Twitter and Reddit), where we assume that they will always reply (i.e. re-enter to the previous conversation) if they receive the notification. \xingshan{add a baseline.}

For supervised models, we compare with \textsc{CCCT}, the state-of-the-art method proposed by \citet{DBLP:conf/wsdm/BackstromKLD13}, where the bagged decision tree with manually-crafted features (including arrival patterns, timing effects, most related terms, etc.) are employed for re-entry prediction. We do not compare with \citet{budak2013participation}, since most of its features are related to social networks or Twitter group information, which is unavailable in our data. %\lu{name the features} 

% \xingshan{neural models have changed.}
In our proposed neural framework, we further compare varying encoders for turn modeling and mechanisms to model the interactions between user history and conversation context.
%For our proposed neural models, 
We first compare three turn encoders --- \textsc{Avg-Embed} (average embedding), \textsc{CNN}, and \textsc{BiLSTM}, to examine their performance in turn representation learning. 
Their results are compared on our variant only with context modeling layer and the best encoder (turned out to be \textsc{BiLSTM}) is applied on the full model.
For the interaction modeling layer, we also study the effectiveness of  four mechanisms to combine user history and conversation context --- simple concatenation (\textsc{Con}), attention (\textsc{Att}), memory networks (\textsc{Mem}), and bi-attention (\textsc{BiA}). 

% We use the variant of our model that ignoring user history modeling layer (so that interaction layer is not exploited), to achieve the goal. Next we compare the performance of four different interaction mechanisms -- Concatenation Merging (\textsc{Mer}), Attention (\textsc{Att}), Memory network (\textsc{MEM}), and Bi-attention (\textsc{BiA}) with the best turn encoder. 
%We also compare with popular neural networks that are good fits for our task. 
%Here we consider \textsc{LSTM} and \textsc{BiLSTM}, both fed with the conversation context in word sequence form extracted from the chronologically ordered turns. 
%We also adapt end-to-end memory networks~\cite{sukhbaatar2015end}, namely \textsc{MemN2N}. It encodes both conversation context and user history for re-entry modeling. To make predictions, a linear layer activated by a sigmoid function is followed, mapping final outputs to predictions, for all above three neural models.
%For model parameters, we apply the same settings as our model, including embeddings, hidden dimensions, batch size, and learning process. And we set hop numbers to be $3$ in \textsc{MemN2N}. 
%\lu{what about model parameters, are they the same as our models? if so, which part?}
%\xingshan{have added some details.}



%\jing{I'm here}

% \subsection{Datasets}

% We design to use two datasets from different platforms, Twitter and Reddit, for experiments. 
% \paragraph{Twitter dataset.}
% We exploit one of datasets in \citet{DBLP:conf/naacl/ZengLWBSW18}, TREC dataset, which is from TREC 2011 microblog track\footnote{\url{https://trec.nist.gov/data/tweets/}} and also for conversation-level task, as our Twitter dataset.
% \paragraph{Reddit dataset [New].}
% %\lu{if this is new, then add [New]}
% This dataset is generated based on a public Reddit comments data provided by a Reddit user\footnote{\url{https://www.reddit.com/r/datasets/comments/3bxlg7/i_have_every_publicly_ available_reddit_comment/}}. The original data contains huge amount of posts and comments available on Reddit from 2006 to 2015. Since it is such a huge amount of content, we focus on the posts and comments in the political domain (which can be found according to ``subreddit'' key word) from 2008.1 to 2008.12. To recover the whole conversations, we use ``parent\_id'' key word to recursively find the parent turn of each comment, until the root of the conversation. Also, we remove those conversations with unknown authors or only containing just one turn (which cannot be called a conversation).

% In our experiments, we predict whether a user will return to a conversation that they has replied, given his first entry in that conversation and all the turns before, and his chatting history of other conversations. Therefore, given a conversation, we will have different conversation-user pair based on the amount of users that has participated in, with different context structure and chatting history.

% The statistics of the two datasets are shown in Table~\ref{tab:stat}. We also display user's history length (i.e. the amount of posts in chatting history) distribution and conversation's turn amount distribution in Figure~\ref{fig:distribution}. As can be seen, two datasets are very different from each other. Reddit dataset is much larger, and users in it tend to take part in more conversations. 
% %(which can be found by statistic of user's history length)
% However, conversations in Twitter dataset last longer in average, and users in it are more likely to return to previous discussions. On the other hand, the same point is, both datasets are imbalanced in some extent, i.e., the amount of positive samples (re-entry) is smaller than that of negative samples (not re-entry). The fact reflects the true situation of real world. Therefore, we choose to use a weighted loss function as our objective function.


% \subsection{Data Preprocessing}
% For preprocessing, we keep all words and punctuations since they may be important for modeling user's behaviors or replying habits. For example, Some combination of punctuations may express emotions of user, like ``:)'' means smiling face. For Reddit dataset, We replace the links with ``URL'' symbols and remove the non-alphabetic tokens. For Twitter dataset, since we will use pre-trained embedding vectors trained by GloVe \cite{pennington2014glove}, we use the preprocessing operation provided by the author of GloVe\footnote{\url{https://nlp.stanford.edu/projects/glove/preprocess-twitter.rb}} to preprocess the data.

% \subsection{Evaluation Metrics and Comparisons}
% Since our work is a binary prediction task, we report the popular metrics AUC and F1-score. While in our experiments, the label distribution is imbalanced, and figuring out the positive samples is more important, so we also report the precision and recall, instead of accuracy.

% For comparison, we compare our method with two simple baselines, a state-of-the-art conventional method, and several neural network based methods.
% \paragraph{Baselines.} For the baselines, one is to randomly classify the given instances (\textsc{RANDOM}); another is to always assign the given instances to be positive, which may be the default method for most current social media platforms (\textsc{NAIVE}).
% \paragraph{Conventional Method.} One of the comparing method (\textsc{CCCT}) is a conventional state-of-the-art method proposed in \citet{DBLP:conf/wsdm/BackstromKLD13}. This method apply bagged decision trees to classify the given instances, by extracting task-specific features including arrival patterns, timing effects, most related terms, etc. We haven't compared with the method in \citet{budak2013participation}, since it is specific for Twitter platform and exploit a lot of Twitter-specific features which are not available in our datasets.
% \paragraph{Neural Network based Methods.} We select most popular RNN-based method -- LSTM \cite{hochreiter1997long} to model the given conversations and predict the task (\textsc{LSTM}). And also try the bidirectional LSTM \cite{graves2005framewise} to see if the performance will be improved (\textsc{BiLSTM}). This two methods can only model the conversations, but hard to process chatting history. So we also employ End to End Memory Network \cite{sukhbaatar2015end} to fit in our task and give the predictions, by treating chatting history as memories, and given conversation as query (\textsc{MEMN2N}).

% \subsection{Training Details}
% We divide our data into three parts: training set, development set and test set, with portions of $80\%$, $10\%$ and $10\%$ respectively. For the neural network based methods, all hyper-parameters are tuned on the development set to obtain the best performance. For batch size, our final choice is $32$. Since we use pre-trained embedding vectors by GloVe \cite{pennington2014glove}, we fix embedding dimension to $200$, and use Twitter-specific pre-trained vectors for our Twitter data, common crawling pre-trained vectors for our Reddit data, respectively. For the hidden state size for LSTM, we set to be $200$ ($100$ for each direction for BiLSTM). We exploit Adam optimization algorithm \cite{kingma2014adam} for model learning, with initial learning rate selected among $\{10^{-3},10^{-4},10^{-5}\}$. Finally, for the weights in loss function, we let $\mu = 1$ and $\lambda = 2$, based on the proportions of true labels.



==> ACL2019(final)/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

%Why we do re-entry prediction?
Interpersonal communication plays an important role in information exchange and idea sharing in our daily life. 
We are involved in a wide variety of dialogues every day, ranging from kitchen table conversations to online discussions, all help us make decisions, better understand important social issues, and form personal ideology. 
However, individuals have limited attentions to engage in the massive amounts of online conversations. There thus exists a pressing need to develop automatic conversation management tools to keep track of the discussions one would like to keep engaging in. 
To meet such demand, we study the problem of {\it predicting online conversation re-entries}, where we aim to forecast whether the users will return to a discussion they once entered.

What will draw a user back?
To date, prior efforts for re-entry prediction mainly focus on modeling user’s engagement patterns in the ongoing conversations~\cite{DBLP:conf/wsdm/BackstromKLD13} or rely on the social network structure~\cite{budak2013participation}, largely ignoring the rich information in users' previous chatting history. 

% Online conversations play an important role in opinion exchange and idea sharing in our daily life. We are involved, actively or passively, in a wide variety of such conversations every day, ranging from chitchats forming the personal ideology to public discussions concerning social issues.
% For individuals, having limited attentions yet facing massive conversations, there exists a pressing need for the conversation management technique to track the engaging discussions one will keep involved. 
% To meet such demand, we study the problem of re-entry prediction, which forecasts whether users will come back to a conversation they once engage in.
% To date, most previous efforts in  the prediction of user re-entries have focused on the modeling of user engagement patterns in the ongoing conversation context~\cite{DBLP:conf/wsdm/BackstromKLD13} and the social network features~\cite{budak2013participation}, while the rich information in users' chatting history have nevertheless been ignored.


% most previous efforts in the related field have focused on the modeling of either the user engagement patterns in conversations~\cite{DBLP:conf/wsdm/BackstromKLD13,jiao2018find} or the interests of users for  recommendation applications~\cite{chen2012collaborative,hong2013co}, while the chatting history of a user has never been explored for learning  for predicting the re-entry behaviors of individuals.

\input{figs/intro-example.tex}

%why conversation context and user history are both useful
Here we argue that effective prediction of one's re-entry behavior requires the understanding of both the \textbf{conversation context}---what has been discussed in the dialogue under consideration, and \textbf{user chatting history} (henceforth user history)---what conversation topics the users are actively involved in. 
In Figure \ref{fig:intro-example}, we illustrate how the two factors together affect a user's re-entry behavior.
Along with two conversations that user $\bf{U_1}$ participated in, also shown is their chatting history in previous discussions. $\bf{U_1}$ comes back to the second conversation since it involves topics on movies (e.g. mentioning \textit{Memento} and \textit{Inception}) and thus suits their interests according to the chatting history, which also talked about movies. 

%As can be seen, $\bf{U_1}$ only re-engaged in the second conversation, concerning two films -- Memento and Inception. It might because these two films fit the interests of $\bf{U_1}$ in thrillers, which can be reflected by $\bf{U_1}$'s preference for a popular thriller Let Me In (LMI) as shown in the chatting history. With limited attention, $\bf{U_1}$ abandoned the first conversation, which focuses on the Oscar event rather than some typical films suiting $\bf{U_1}$'s special tastes.

%Our model
%\xingshan{changed some descriptions to fit in our new point.}
In this work, we would like to focus on the joint effects of conversation context and user history, ignoring other information. It would be a more challenging yet general task, since information like social networks may be not available in some certain scenarios. 
To study how conversation context and user history jointly affect user re-entries, we propose a novel neural framework that incorporates and aligns the indicative representations from the two information source.
To exploit the joint effects, four mechanisms are employed here:
%\textbf{Simple Concatenation} 
\emph{simple concatenation} of the two types of representation, \emph{attention} mechanism over turns in context, %merely drawing user-aware context representation; 
%what's the difference between this and bi-attn? make it clearer, it doesn't have to be long, can be very short phrases, but reviewers will quickly know what's going on}, 
\emph{memory networks}~\cite{sukhbaatar2015end} --- able to learn context attentions in aware of user history,
%, treating user history as memory modules and passing context through them; 
and \emph{bi-attention} \cite{seo2016bidirectional} --- further capturing interactions from two directions (context to history and history to context). 
%\jing{Updated.}
%\lu{basically, you need a summary of the mechanisms here since comparison becomes a major contribution}
% Concretely, we propose a novel neural framework for predicting online conversation re-entries with different mechanisms ( including \textbf{MemN2N} \cite{sukhbaatar2015end} and \textbf{bi-attention} \cite{seo2016bidirectional}) to incorporate and align the indicative representations from the conversation context and the user history. 
More importantly, our framework
%\lu{models? now each of them is a model right, or you want to say framework?} 
enables the re-entry prediction and corresponding representations to be learned in an end-to-end manner. 
On the contrary, previous methods for the same task rely on handcrafted features~\cite{DBLP:conf/wsdm/BackstromKLD13,budak2013participation}, which often require labor-intensive and time-consuming feature engineering processes. 
%In a similar task of conversation recommendation~\cite{DBLP:conf/naacl/ZengLWBSW18}, Bayesian models are applied to induce latent representations, where domain knowledge is unavoidably involved to customize the model inference algorithms. 
To the best of our knowledge, we are the first to explore the joint effect of conversation context and user history on predicting re-entry behavior in a neural network framework. 

% Most existing methods, however, applies hand-coded features~ or latent representations induced by topic models~\cite{DBLP:conf/naacl/ZengLWBSW18}, and hence relies on the expertise involved to customize the feature design or the model inference algorithms. \lu{can you say more about previous work on this task, or what is the SOTA?}

%Empirical studies
We experiment with two large-scale datasets, one from Twitter~\cite{DBLP:conf/naacl/ZengLWBSW18}, the other from Reddit which is newly collected\footnote{The datasets and codes are released at: \url{https://github.com/zxshamson/re-entry-prediction}}. Our framework with bi-attention significantly outperforms all the comparing methods including the previous state of the art~\cite{DBLP:conf/wsdm/BackstromKLD13}. For instance, our model achieves an F1 score of $61.1$ on Twitter conversations, compared to an F1 score of $57.0$ produced by \citet{DBLP:conf/wsdm/BackstromKLD13}, which is based on a rich set of handcrafted features. 
%
Further experiments also show that the model with bi-attention can consistently outperform comparisons given varying lengths of conversation context.
It shows that bi-attention mechanism can well align users' personal interests and conversation context in varying scenarios.
%over other mechanisms. 
%\xingshan{Added words to show the comparison of different mechanisms.}

After probing into the proposed neural framework with bi-attention, we find that meaningful representations are learned via exploring the joint effect of conversation context and user history, which explains the effectiveness of our framework in predicting re-entry behavior. 
%
Finally, we carry out a human study, where we ask two humans to perform on the same task of first re-entry prediction. The model with bi-attention outperforms both humans, suggesting the difficulty of the task as well as the effectiveness of our proposed framework. 
%while models can exhibit better results by learning useful representations from large data. 

% In experiments, we evaluate our proposed model on two large-scale datasets, a publicly available one from Twitter and a newly collected one from Reddit.\footnote{Dataset will be released upon publication.} The comparison results with the existing models show that our model exhibits the best performance in re-entry prediction. For example, we achieve $60.6$ F1 score on Twitter, better than the state-of-the-art results of $57.0$ produced by \citet{DBLP:conf/wsdm/BackstromKLD13}.
% Further analysis shows that our model, that effectively explores the user chatting history, can consistently outperform comparison models given varying length of conversation context. 
% We then present more studies on our model and the results show that meaningful representations are learned via exploring the joint effects of conversation context and user history, which explains the superiority of our model in predicting re-entry behaviors.
% A human evaluation is further presented showing that re-entry prediction is challenging even for humans, while models can exhibit better results by learning useful representations from large data. 



==> ACL2019(final)/sections/model.tex <==
%\section{Our Neural Model with Bi-Attention for Re-entry Prediction}
\section{Neural Re-entry Prediction Combining Context and User History}

This section describes our neural network-based conversation re-entry prediction framework exploring the joint effects of context and user history.
%which is designed with different interaction mechanism over the conversation context and user history. 
Figure \ref{fig:mod} shows the overall architecture of our framework, consisting of three main layers: context modeling layer, user history modeling layer, and interaction modeling layer to learn how information captured by the previous two layers interact with each other and make decisions conditioned on their joint effects.
Here we adopt four mechanisms for interaction modeling: simple concatenation, attention, memory networks, and bi-attention, which will be described later. 
%on whether the user will return to the previously involved conversation. 

%Bi-attention mechanism is first proposed for the task of reading comprehension~\cite{seo2016bidirectional}, and has proven useful in text classification tasks~\cite{zhou2016attention,bai2018deep}. Our work is the first to exploit this mechanism for conversation modeling. 

%\xingshan{Bi-attention mechanism is first proposed for task of reading comprehension~\cite{seo2016bidirectional}, and has been proved to be useful in different classification tasks~\cite{zhou2016attention,bai2018deep}. Our work is first to exploit such mechanism in conversation-level task.}

%one for context modeling, one for user history modeling, and the other with the bi-attention mechanism for combining what is captured by the previous two layers and makes the prediction on whether the target user will return to the target conversation.

\input{figs/framework.tex}

\subsection{Input and Output}\label{ssec:model:io}
We start with formulating model input and output. At input layer, our model is fed with two types of information, the chatting history of the target user $u$ and the observed context of the target conversation $c$. 
The goal of our model is to output a Bernoulli distribution $p(u,c)$ indicating the estimated likelihood of whether $u$ will re-engage in the conversation $c$. Below gives more details.
%for the input.

%\xingshan{add some description for input of context and history.}
Formally, we formulate the context of $c$ as a sequence of chronologically ordered turns $\langle t_1,t_2,\cdots,t_{|c|}\rangle$, where the last turn $t_{|c|}$ is posted by $u$ (we then predict $u$'s re-entries afterwards). 
%, which includes the posts of current conversation $c$ until user $u$'s first entry (if predicting the first re-entry). 
%\jing{Updated the wordings.}
%where $|c|$ is the number of turns in $c$'s context. 
%Each turn $t$ has two sequences to represent it: a sequence of words observed in $t$, ${\bf w}_t$, and an auxiliary triple, ${\bf a}_t$, conveying some of $t$'s meta information. 
Each turn $t$ is represented by a sequence of words ${\bf w}_t$, and an auxiliary triple, ${\bf a}_t=\langle i_{t}, r_{t}, u_{t}\rangle$, 
%with $t$'s meta information. 
%Specifically, ${\bf w}_t=\langle w_{t,1}, w_{t,2}, \cdots, w_{t,|t|}\rangle$, with $|t|$ denoting the number of words in $t$. 
%
%The auxiliary triple takes a form of ${\bf a}_{t}=\langle i_{t}, r_{t}, u_{t}\rangle$, 
where $i_{t}$, $r_{t}$, and $u_{t}$ are three indexes indicating the position of turn $t$, which turn $t$ replies to, and the author of $t$, respectively. 
Here ${\bf a}_{t}$ is used to record the replying structures as well as the user's involvement pattern. 
%and the target user's activities. %in conversation context.

For the user history, we formulate it as a collection of $u$'s chatting messages $\{m_1, m_2, \cdots, m_{|u|}\}$, all posted before the time $t_{|c|}$ occurs.
%(until the first entry of current conversation if predicting the first re-entry)
%($|u|$ refers to the count of messages in $u$'s user history). 
Each message $m$ is denoted as its word sequence, ${\bf w}_m$. %\jing{Updated the wordings.}
%=\langle w_{m,1}, w_{m,2}, \cdots, w_{m,|m|}\rangle$, with $|m|$ representing its word count.

In the following, we explain how the aforementioned representations are processed by our model to make predictions. 
The three main layers in Figure~\ref{fig:mod} are described in Sections \ref{ssec:model:context}, \ref{ssec:model:user}, and \ref{ssec:model:bi-attention}, respectively. The learning objective is presented in Section \ref{ssec:model:final}. 




\subsection{Context Modeling Layer}\label{ssec:model:context}

The context modeling layer captures representations from the observed context for the target conversation $c$. 
To this end, we jointly model the content in each turn (henceforth \textbf{turn modeling}) and the turn interactions in conversation structure (henceforth \textbf{structure modeling}). 
%Here we present two bidirectional long-short term memory (BiLSTM) models in a hierarchical structure, one for each components. 
%one for turn modeling and the other for structure modeling. We describe them in turn below.

\paragraph{Turn Modeling.} 
The turn representations are modeled via turn-level word sequence with a turn encoder. 
We exploit three encoders here: \textbf{Average Embedding} (Averaging each word's embedding representation), \textbf{CNN} (Convolutional Neural Networks), and \textbf{BiLSTM} (Bidirectional Long Short-Term Memory).
BiLSTM's empirical performance turns out to be slightly better (will be reported in Table~\ref{tab:main_res}).
% The experimental results (Table~\ref{tab:main_res}) show that BiLSTM performs slightly better than the other two encoders.

Concretely, given the conversation turn $t$, each word $w_i$ of $t$ is represented as a vector mapped by an embedding layer $I(\cdot)$, which is initialized by pre-trained embeddings and updated during training. %\lu{which embedding is used? maybe add here?}
The embedded vector $I(w_i)$ is then fed into the turn encoder, yielding the \textit{turn representation} for $t$, denoted by $H^T_{t}$.\footnote{For all the BiLSTM encoders in this work, without otherwise specified, we take the concatenation of all hidden states from both the directions as its learned representations.}
%As BiLSTM has two opposite directions, the turn representation of $t$, denoted by $H^T_{t}$, takes the concatenation all the hidden states in BiLSTM.


\paragraph{Structure Modeling.} 
To learn the conversational structure representations for $c$, our model applies BiLSTM, namely structure encoder, to capture the interactions between adjacent turns in its context.  
Each state of this structure encoder sequentially takes $t$'s turn representation, $H_{t}^T$, concatenated with the auxiliary triple, ${\bf a}_t$, as input to produce the structure representation $H^C$. 
Our intuition is that $H^C$ should capture both the content of the conversation and interaction patterns among its participants.  
%\xingshan{(so that the tree structure and user activity of conversations can be captured by the model)}, and produce the structure representation $H^C$. 
Then $H^C$, considered as the \textit{context representation} for $c$, is sent to interaction modeling layer as part of its input. % for further processing. 
%And similar to the turn modeling, we concatenate all the hidden states from both directions of the BiLSTM for structure modeling and yield $H^C$, conveying context representations for $c$.


\subsection{User History Modeling Layer}\label{ssec:model:user} 
To encode the user history for target user $u$, in this layer, we first apply the same encoder in turn modeling to encode each chatting message $m$ by $u$, as they both explore the post-level representations.
The turn encoder is sequentially fed with the embedded word in $m$, and produce the message-level representation $H^M_m$. All messages in $u$'s user history are further concatenated into a matrix $H^U$, serving as $u$'s \textit{user history representation} and the input of the next layer.

\subsection{Interaction Modeling Layer}\label{ssec:model:bi-attention}

To capture whether the discussion points in $c$ match the interests of $u$,  
$H^C$ (from context modeling) and $H^U$ (from user history modeling) are merged through an interaction modeling mechanism over the two sources of information.
%bidirectional attention (bi-attention) mechanism over the sources of information. 
We hypothesize that users will be likely to come back to a conversation if its topic fits their own interests. 
%Our assumption is that what draws a user back to a conversation might be some topics discussed there fitting the user's interests. 
%In this situation, there will be similar content appearing
Here, we explore four different mechanisms for interaction modeling.
Their learned interaction representation, denoted as ${\bf r}^O$, is fed into a sigmoid-activated neural perceptron~\cite{glorot2011deep}, for predicting final output $p(u,c)$. 
It indicates how likely the target user $u$ will re-engage in the target conversation $c$. 
We then describe the four mechanisms to learn ${\bf r}^O$ in turn below.

%or our model, hoping to find a best method to model the interactions between context and user history.

\paragraph{Simple Concatenation.} 
% An intuitive simple mechanism is to directly concatenate the two representations derived from the last two layers.
% This mechanism is easy to implement, but may be not able to capture useful information for prediction.
Here we simply put context representation (last state) and user representations (with average pooling) side by side, yielding ${\bf r}^O=[H^C_{|c|}; \sum_j^{|u|} H^U_j / |u|]$ as the interaction representation for re-entry prediction.

\paragraph{Attention.} 
To capture the context information useful for re-entry prediction, we exploit an attention mechanism~\cite{luong2015effective} over $H^C$.
Attentions are employed to ``soft-address'' important context turns according to their similarity with user representation (with average pooling). 
Here we adopt dot attention weights and define the attended interaction representation as:
\vspace{-1mm}
\begin{equation}\small
    {\bf r}^O= \sum_i^{|c|} \alpha_{i}\cdot H^C_i\text{, } \alpha_{i}=softmax(H_i^C\cdot \sum_j^{|u|} H^U_j/{|u|})
    \vspace{-1mm}
\end{equation}

\paragraph{Memory Networks.}

To further recognize indicative chatting messages in user history, we also apply end-to-end memory networks (MemN2N)~\cite{sukhbaatar2015end} for interaction modeling.
It can be seen as a recurrent attention mechanism over chatting messages (stored in memory).
Hence fed with context representation, memory networks will yield a memory-aware vector as interaction representation:
\vspace{-2mm}
\begin{equation}\small \label{mem}
    {\bf r}^O= \sum_j^{|u|} \alpha_{j}\cdot f_{turn}(H^U_j)\text{, } \alpha_{j}=softmax(H^C_{|c|}\cdot H^U_j )
    \vspace{-2mm}
\end{equation}
\noindent where $f_{turn}(\cdot)$ denotes the unit function used for turn modeling.
%means turn encoder with different parameters from aforementioned.
%${\bf r}^I = H^C_{|c|}$.

Here we adopt multi-hop memory mechanism to allow deep user interests to be learned from chatting history. For more details, we refer the readers to \citet{sukhbaatar2015end}. 
%This means that Eq.~\ref{mem} is applied multiple times, while in each time, we have ${\bf r}^{I,n+1} = {\bf r}^{O,n} + {\bf r}^{I,n}$.

\paragraph{Bi-attention.}
Inspired by~\citet{seo2016bidirectional}, we also apply bi-attention mechanism to explore the joint effects of context and user history.
Intuitively, the bi-attention mechanism looks for evidence, if any, indicating the topics of the current conversation that align with the user's interests from two directions (i.e. context to history and history to context), such as the names of two movies \textit{Inception} and \textit{Let Me In} shown in Figure \ref{fig:intro-example}. Concretely, bi-attention mechanism captures context-aware attention over user history messages:
%\vspace{-1mm}
\begin{equation}\small
\alpha^U_{ij}=\frac{\exp(f_{score}(H^C_i,H^U_j))}{\sum_{j'=1}^{|u|} \exp(f_{score}(H^C_i,H^U_{j'}))}
%\vspace{-1mm}
\end{equation}
%
\noindent where the alignment score function takes a form of $f_{score}(H^C_i,H^U_j)= W_{bi-att}[H^C_i;H^U_j;H^C_i \circ H^U_j]$. 
It captures the similarity of the $i$-th context turn and the $j$-th user history message. The weight vector $W_{bi-att}$ is learnable in training.

Likewise, we compute user-aware attention over context turns.
Afterwards, the bi-directional attended representations are concatenated and passed into a ReLU-activated multilayer perceptron (MLP), yielding representation $\bf r$.
%~\cite{glorot2011deep}.  %For more details, we refer the readers to \citet{seo2016bidirectional}.
$\bf r$, as turn-level representation, is then sequentially fed into a two-layer BiLSTM, to produce the interaction representation ${\bf r}^O$. 



% We treat user history as memory module, and then input the context representation to get the memory-aware final representation, with multiple hops of computation. Each hop will store and update the memory module, so the final output can possibly reflect more about user's interests.

%\jing{I'm here.}

% Attention mechanism~\cite{luong2015effective} can be exploited upon Structure Modeling part, to form the history-aware representation of the conversation. To draw the attended representation, we first compute the similarities between representations of context and user history, using dot product. And then a softmax function is used among the computed similarities to draw attention weights for each turn. The final attended representation will be the weighted sum of each turn's representation.

% \paragraph{Memory Network.}
% End-to-end memory networks (MemN2N)~\cite{sukhbaatar2015end}, can be seen as a recurrent attention model over external memory. We treat user history as memory module, and then input the context representation to get the memory-aware final representation, with multiple hops of computation. Each hop will store and update the memory module, so the final output can possibly reflect more about user's interests.

% \paragraph{Bi-attention.}
% Inspired by~\citet{seo2016bidirectional}, we also apply bi-attention mechanism to see if we can find more efficient representations for prediction. 
% Intuitively, the bi-attention mechanism looks for evidence, if any, indicating the topics of the current conversation that align with the user's interests from two directions (i.e. context to history and history to context), such as the names of two movies \textit{Inception} and \textit{Let Me In} shown in Figure \ref{fig:intro-example}. In bi-attention mechanism, our model tries to capture two directional attention weights -- context-aware attention and user-aware attention by a tailored similarity computing method. And then the two directional attention are combined and passed into a ReLU activated multilayer perceptron (MLP)~\cite{glorot2011deep}, followed by a two-layer BiLSTM, to produce final representation output (Due to the space limitation, please refer to \citet{seo2016bidirectional} for more details).
% \xingshan{It seems that reviewers not very care about the details of our model, so I think we can omit some details .}

%Intuitively, the bi-attention mechanism looks for evidence, if any, indicating the topics of the current conversation that align with the user's interests, such as the names of two movies \textit{Inception} and \textit{Let Me In} shown in Figure \ref{fig:intro-example}.  This mechanism is inspired by~\citet{seo2016bidirectional} and tailored for our task.
%
%Concretely, we put a \textit{context-aware attention} on $H^U$ (produced by the user history modeling layer) to identify the messages in $u$'s chatting history focusing on similar topics in the conversation. Its attention weights are computed as follows:
%
%\vspace{-1mm}
%\begin{equation}\small
%\alpha^U_{ij}=\frac{\exp(f_{score}(H^C_i,H^U_j))}{\sum_{j'=1}^{|u|} \exp(f_{score}(H^C_i,H^U_{j'}))},
%\end{equation}
%
%\noindent where the alignment score function takes a form of $f_{score}(H^C_i,H^U_j)= W_{bi-att}[H^C_i;H^U_j;H^C_i \circ H^U_j]$. It captures the similarity of the $i$-th turn in context and the $j$-th message in user history. The weight vector $W_{bi-att}$ is learnable in training. 
%We then compute an attended matrix $R^U$ as the \textit{context-aware user representation}. The $i$-th row indicates the representation that reflects similarities between $u$'s past messages and the $i$-th turn in $c$. It is defined as:
%
%\vspace{-1mm}
%\begin{equation}\small
%R^U_i=\sum_{j=1}^{|u|}\alpha^U_{ij}H^U_j.
%\end{equation}
%
%Similarly, we learn a \textit{user-aware attention} over the context representations $H^C$, with coefficient $\alpha^C$ and the attended matrix $R^C$ as the \textit{user-aware context representation}. 
%Here each column in $R^C$ conveys the salient points exhibited by each turn in conversation $c$'s context that suits the interests of user $u$.
%
%To combine $R^U$ and $R^C$, we first conduct max pooling on each column in $R^C$, yielding a vector ${\bf r}^C$, as done in \citet{seo2016bidirectional}. 
%${\bf r}^C$ is then concatenated with each row in $R^U$ and $H^C$ (structure representation derived in context modeling layer), to be passed into a ReLU activated multilayer perceptron (MLP)~\cite{glorot2011deep}. This forms the combined turn representation $\bf r$. 
%Afterwards, $\bf r$, with  representations captured at turn level, is sequentially fed into a two-layer BiLSTM, to produce final representation output ${\bf r}^O$. %of the whole procedure. 

% To give the final prediction, a linear layer, activated by a sigmoid function, is exploited on ${\bf r}^O$ (the final representation output of aforementioned interaction mechanisms) to produce the output $p(u,c)$, which indicates how likely the target user $u$ will re-engage in the target conversation $c$. 

\subsection{Learning Objective}\label{ssec:model:final}

For parameter learning in our model, we design the objective function based on cross-entropy loss as following:

\vspace{-2mm}
\begin{equation} \label{loss}
\small
\mathcal{L} = - \sum_i \big [ \lambda y_i \log (\hat{y}_i) + \mu (1 - y_i) \log (1 - \hat{y}_i) \big ]
\vspace{-2mm}
\end{equation}
%
\noindent where the two terms reflect the prediction on positive and negative instances, respectively.
Moreover, to take the potential data imbalance into account, we adopt two trade-off weights $\lambda$ and $\mu$. %, to balance the fitting on positive and negative instances. 
The parameter values are set based on the proportion of positive and negative instances in the training set (see Section~\ref{sec:expsetup}). 
%For the values of $\lambda$ and $\mu$, they are set based on the proportion of positive and negative instances in true datasets.
$\hat{y}_i$ denotes the re-entry probability estimated from $p(u,c)$ for the $i$-th instance, %(formed by a target conversation $c$ and a target user $u$), 
and $y_i$ is the corresponding binary ground-truth label ($1$ for re-entry and $0$ for the opposite).
%\lu{for lambda and mu, if use the same values for experiments, mention them here; if not, say something like they're tuned for different datasets on the development set}


%\jing{I'm here!}

% The input of our model includes the conversation $C=\{c_1,c_2,...,c_t\}$ that a user $U$ has replied before, and the chatting history of the giving user $H=\{h_1,h_2,...,h_s\}$ ($t$ and $s$ are the post amount for conversation and history respectively). 
% Each turn $c_i$ contains the words $\{x_{i_1},x_{i_2},...,x_{i_l}\}$ and the context information $T_i$ (including turn ID, turn ID of its father, user ID). And each chatting history $h_j$ is a post that the user has published before, only containing the words $\{x_{j_1},x_{j_2},...,x_{j_m}\}$. 
% %\lu{it's confusing that l is used twice for ci and hj, not explained}
% The output of our model will be the probability that the giving user will re-enter the conversation.
% %\lu{it's confusing that what makes a reply history, hj, is it a post? if so, explain it clearly. maybe change "reply history" to "post history or chat history", since reply will be used in current conversation too}
% \xingshan{Have changed ``reply history'' to ``chatting history'', consistent with the description in intro.}

% Basically our model contains two encoding layers to model the conversation and user's history, respectively. And then a Bidirectional attention layer \cite{seo2016bidirectional} is used to connect these two layers and produce attended feature vectors of the conversation, following by an output layer to provide the final prediction. Figure~\ref{fig:mod} displays the overall model.


% \subsection{Conversation Modeling Layer}
% To better model the content and structure of the whole conversation, we choose to use a hierarchical multi-layers Bidirectional LSTM (BiLSTM) \cite{graves2005framewise} to encode the conversation.

% For each turn of the conversation, we first use an embedding layer, which has been pre-trained using GloVe \cite{pennington2014glove}, to map each word $x_{ij}$ to a high-dimensional vector $\boldsymbol{x}_{ij}$. And then a one-layer BiLSTM is used to model the temporal interactions between words (We name the combination of the embedding layer and BiLSTM layer ``Post Modeling'' for convenience), and the output $\boldsymbol{X}_{i}$ will be the vector representation of current turn, together with context information $T_i$, i.e.,
% %\lu{X is not in fig 2}
% \begin{equation} \label{turn_rep}
% \boldsymbol{C}_i = [\boldsymbol{X}_i;T_i]
% \end{equation}
% where ``$[;]$'' means concatenating operation, and $i$ means the $i$-th turn of current conversation.
% %\lu{here I forget about i, so need to reminder readers, Ti is not bold, so it's real value? but it's a vector right?}
% \xingshan{Ti stores turn ID, father's turn ID and user ID, which together can reflect tree structure of the conversation. I am not sure whether it should be bold or not.}

% Having the vector representation of each turn, we finally use a stacked BiLSTM to model the whole conversation (The number of recurrent layers will be the parameter to be tuned). The output will be a matrix $\boldsymbol{C} \in \mathbb{R}^{t \times d}$ containing each turn's final representation, where $t$ is the number of turns and $d$ is hidden dimension. 

% \subsection{User's History Modeling Layer}
% User's chatting history (User's history for short later) contains the posts that the user has published before. Since there is no structural information among these posts, and temporal effect is not so distinct, we decide not to model the ordering of history posts. We only use the same Post Modeling layer (i.e. embedding layer and one-layer BiLSTM) that in last subsection, to model the words of each post. By combining the vector representations of history posts, matrix $\boldsymbol{H} \in \mathbb{R}^{s \times d}$ is constructed to represent the user's history, where $s$ is the number of history messages.

% \subsection{Bidirectional Attention Layer}
% Inspired by \citet{seo2016bidirectional}, we use a Bidirectional attention flow to enhance the connection between conversation content and history posts, hoping to find out the most relevant turn and history, which can reflect user's behaviors and so that decisive for prediction. \xingshan{have changed the description}
% %decisive turn content \lu{a bit awkward} that is most relevant to user's history behaviors. 
% Therefore, the first step will be computing similarities between conversation content and history messages. We use the following equation to compute the similarity between turn $\boldsymbol{C}_i$ and history $\boldsymbol{H}_j$:
% \begin{equation} \label{sim}
% \boldsymbol{S}_{ij} = \boldsymbol{W}_{\boldsymbol{S}}^T [\boldsymbol{C}_i;\boldsymbol{H}_j;\boldsymbol{C}_i \circ \boldsymbol{H}_j] 
% \end{equation}
% where $\boldsymbol{W}_{\boldsymbol{S}} \in \mathbb{R}^{3d}$ is a weight vector that can be trained, and $\circ$ is pointwise multiplication.

% With the similarity matrix, attention for two directions can be computed according to the following equations:
% \begin{equation} \label{c2h}
% \hat{\boldsymbol{H}}_i = \sum_j a_{ij} \boldsymbol{H}_j
% \end{equation}
% \begin{equation} \label{h2c}
% \hat{\boldsymbol{C}} = \sum_i b_{i} \boldsymbol{C}_i
% \end{equation}
% where $\hat{\boldsymbol{H}}_i$ is conversation-to-history attended vector for turn $i$, reflecting the most relevant history message of turn $i$; $\hat{\boldsymbol{C}}$ is history-to-conversation attended vector, indicating the weighted sum of the most important turns with respect to history; and $a_i = softmax(\boldsymbol{S}_{i:})$, $b = softmax(max_{col}(\boldsymbol{S}))$ are the attention weights for two directions.\lu{the notations are informal above, e.g. max, col, need to rework on the explantion above, alpha is awkward usage, use f or g or something lke a function to indicate MLP}
% \xingshan{The notations of $max_{col}$ are learnt from \citet{seo2016bidirectional}, I haven't think of a better way to describe it....}

% Finally, these two attended vectors are combined together to yield history-aware representation of each turn of the conversation $\tilde{\boldsymbol{C}}_i$. We decide to use two-layer MLP activated with ReLU \cite{glorot2011deep} over the concatenation of several representations to compute this final representation. The equation is as follow:
% \begin{equation} \label{mlp}
% \tilde{\boldsymbol{C}}_i = f_1(f_2( [\boldsymbol{C}_i;\hat{\boldsymbol{H}}_i;\boldsymbol{C}_i \circ \hat{\boldsymbol{H}}_i;\boldsymbol{C}_i \circ \hat{\boldsymbol{C}}]))
% \end{equation}
% where $f_*$ means an MLP layer. Recall that $\boldsymbol{C}_i$ and $\hat{\boldsymbol{H}}_i$ are vector representation and conversation-to-history attended vector for turn $i$ respectively, and $\hat{\boldsymbol{C}}$ is history-to-conversation attended vector.
% %\lu{up to here readers forget about what are the notations above, need to remind them or think about better display}

% \subsection{Output Layer}
% To give the final prediction, we first use a multi-layer stacked BiLSTM to model the outputs of last layer, $\tilde{\boldsymbol{C}}_i$, which are history-aware representations of those turns in the conversation. The result of such BiLSTM is noted as $\boldsymbol{C}_O$. Since our task is a binary classification, the final output layer will be a linear layer followed by a sigmoid function, to produce final output $\hat{y}$ with value in $[0,1]$, which considered as probability that the given user will re-enter the given conversation.
% \begin{equation} \label{output}
% \hat{y} = Sigmoid( \boldsymbol{W}_O^T \cdot \boldsymbol{C}_O + b)
% \end{equation}

% \subsection{Loss Function}
% We use weighted binary cross entropy loss to train our model. Therefore, the objective will be minimizing the following loss function:
% \begin{equation} 
% \small
% \mathcal{L} = - \sum_i w_1 y_i \log (\hat{y}_i) + w_0 (1 - y_i) \log (1 - \hat{y}_i)
% \end{equation}
% where $\hat{y}_i$ is the probability of the i-th conversation-user pair that predicted to re-entry, and $y_i$ is the ground-truth label (either 1 or 0). $w_0$, $w_1$ are the weights for negative and positive parts of the loss function respectively, whose function is to tackle the problem of imbalanced data (We will discuss more about it in next section).

==> ACL2019(final)/sections/related_work.tex <==
\section{Related Work}

%Our work is related to two research areas: predicting responses to social media posts and understanding online conversation behavior. 

\paragraph{Response Prediction.} 
Previous work on response prediction mainly focuses on predicting whether users will respond to a given social media post or thread. 
Efforts have been made to measure the popularity of a social media post via modeling the response patterns in replies or retweets~\cite{artzi2012predicting,zhang2015retweet}. 
Some studies investigate post recommendation by predicting whether a response will be made by a given user~\cite{chen2012collaborative,yan2012tweet,hong2013co,alawad2016network}.
%Some predicts the specific response of a certain user for post recommendation~\cite{chen2012collaborative,yan2012tweet,hong2013co,alawad2016network}.

In addition to post-level prediction, other studies focus on response prediction at the conversation-level. \citet{DBLP:conf/naacl/ZengLWBSW18} investigate microblog conversation recommendation by exploiting latent factors of topics and discourse with a Bayesian model, which often requires domain expertise for customized learning algorithms. 
%However, expertise is often required for customizing algorithms in Bayesian model's parameter estimation. 
Our neural framework can automatically acquire the interactions among important components that contribute to the re-entry prediction problem, and can be easily adapted to new domains. 
%However, due to the limitation of most Bayesian models, expertise is required for customizing algorithms in parameter estimation. Our model, however, exhibits better ability in model extension, taking advantages of the neural network framework.  
For the prediction of re-entry behavior in online conversations, previous methods rely on the extraction of manually-crafted features from both the conversation context and the user's social network~\cite{DBLP:conf/wsdm/BackstromKLD13,budak2013participation}. 
Here we tackle a more challenging task, where the re-entries are predicted without using any information from social network structure, which ensures the generalizability of our framework to scenarios where such information is unavailable. 
%which ensures our general applicability in scenarios lacking some specific information. 
%Moreover, our work can be benefited from its neural network architecture that allows the end-to-end training process, while \citet{DBLP:conf/wsdm/BackstromKLD13} relies on an expensive process for feature engineering. 

\paragraph{Online Conversation Behavior Understanding.} 
Our work is also in line with conversational behavior understanding, including how users interact in online discourse~\cite{DBLP:conf/naacl/RitterCD10} and how such behavior signals the future trajectory, including their continued engagement~\cite{DBLP:conf/wsdm/BackstromKLD13,jiao2018find} and the appearance of impolite behavior~\cite{zhang2018conversations}. 
To better understand the structure of conversations, Recurrent Neural Network (RNN)-based methods have been exploited to capture temporal dynamics~\cite{cheng2017factored,DBLP:journals/tacl/ZayatsO18,jiao2018find}. 
Different from the above work, our model not only utilizes the conversations themselves, but also leverages users' prior posts in other discussions.
%Distinguishing from previous work, modeling user behaviors regardless of their interests, we study the re-entry behaviors for a specific user, where the user interests should be learned from the chatting history for prediction.


%\jing{I'm here!}

%\xingshan{Have combined our two versions!}

%Response prediction, whose goal is to predict whether a giving post will receive replying or sharing, has been explored in diverse aspects \cite{artzi2012predicting,zhang2015retweet,yang2017characterizing}. It has been viewed as a classification task, using feature-extracting classification model to classify \cite{artzi2012predicting} or probabilistic graphical model to model the trend and then compute the probability \cite{zhang2015retweet}; or a recommendation task, using graph ranking models \cite{yan2012tweet,alawad2016network} or recommendation-specific methods like collaborative filtering to extract user interests and then do the prediction \cite{chen2012collaborative,hong2013co}.

%Most of social media allow users to reply or give comments to the original posts. Conversations formed by such behaviors may contain rich information, so that more and more researchers focus on tasks of conversation-level\cite{gomez2011modeling,cheng2014can,Cheng:2017:ABT:2998181.2998213}. To model the conversations, topic modeling \cite{DBLP:conf/naacl/RitterCD10,DBLP:conf/naacl/ZengLWBSW18} and RNN-based methods \cite{luan2016lstm,DBLP:journals/tacl/ZayatsO18} which can capture temporal dynamic behaviors for conversations have been exploited in previous work. 

%Among the diverse tasks on conversation-level, our work is most related to engagement prediction, which can be roughly divided to length prediction and re-entry prediction. Length prediction is to predict how long will the giving conversation lasts\cite{DBLP:conf/wsdm/BackstromKLD13,cheng2014can}, including predicting whether the current turn is an ending post \cite{jiao2018find,zhang2018conversations}. Our work is exactly re-entry prediction, which also has been explored in some extent in previous work \cite{DBLP:conf/wsdm/BackstromKLD13,budak2013participation}. However, our work is the first to use neural network model to do the end-to-end prediction, with the consideration of user's reply history as extra features at the same time.

==> ACL2019(final)/sections/result.tex <==

%\section{Experimental Results}
\section{Results and Analysis}
This section first discusses prediction results of first re-entry in Section~\ref{ssec:first-reentry}. 
We then present the results of the second and third re-entry prediction in Section \ref{ssec:context-and-history}, as well as an analysis on user history effects.
%Quantitative and qualitative analysis is provided in 
Section~\ref{ssec:discussion} then provides explanations on what we learn from the joint effects from context and user history, indicative of user re-entries.
%better performance than comparisons. 
%Then in Section \ref{ssec:discussion}, we further explain our superiority from both quantitative and qualitative perspectives.
Finally, we conduct a human study to compare human performance on the same task with our best model (Section~\ref{ssec:human}).
%we compare the performance of human and machines on our task in Section \ref{ssec:human}.

\subsection{First Re-entry Prediction Results}\label{ssec:first-reentry}

\input{tables/comparison.tex}

% We use the metrics of AUC, F1, precision, and recall, for automatic evaluation. 
In main experiment, we adopt the automatic evaluation metrics --- AUC, F1 score, precision, and recall, and focus on the prediction of the major re-entry type --- {\it first re-entry}, where conversation context up to user's first participation is given. 
As shown in Table \ref{tab:stat}, most users, if re-entry, only return once to a conversation. Also, in  conversation management, the prediction of first re-entry is a challenging yet practical problem.
%compared with the other re-entry types.
We will discuss second and third re-entry prediction later in Section \ref{ssec:context-and-history}.
%We hence start with {\it first re-entry prediction}, where conversation context up to user's first participation is given.  
%We first study how models perform on first re-entry prediction, only given the conversation context including the user's first participation, considering that most users in our data engage in a conversation at most twice (as shown in Table \ref{tab:stat}). 
The comparison results 
%on first re-entry prediction 
are reported in Table \ref{tab:main_res}. 
On both datasets, we observe: 

%\lu{the italics and bold are too much, use one is good}
\vspace{0.5em}
%$\bullet$~\textit{Models exhibit different performance on the two datasets.} 

$\bullet$~\textit{First re-entry prediction is challenging}. All models produce AUC and F1 scores below $70$. In particular, models built on rules and features with shallow content and network features perform poorly, suggesting the need of better understanding of conversations or more information like user's chatting history. 
We also observe that \textsc{History} yields only slightly better results than \textsc{Random}.
It suggests that users' re-entries depend on not only their past re-entry patterns, but also the conversation context.
%We found tly hat all models produce AUC and F1 scores below $70$. Non-neural methods, particularly, work poorly, indicating that it is not possible to rely on simple rules or hand-coded features to effectively predict conversation re-entries.

% $\bullet$~\textit{BiLSTM is the best turn encoder}. Not surprisingly, Average Embedding performs poorest among the proposed three turn encoder, since it cannot capture the information of word position. And BiLSTM performs better than CNN, this indicates that BiLSTM handles better than CNN on modeling such short messages of turns in Online conversations. \xingshan{Add a point for discussing turn encoders.}

$\bullet$~\textit{Well-encoded user chatting history is effective.} 
%\xingshan{changed due to new variant's performance.}
Among neural models, our \textsc{BiLSTM+Mem} and \textsc{BiLSTM+BiA} models outperform other comparisons by successfully modeling users' previous messages and their alignment with the topics of ongoing conversations. 
However, the opposite observation is drawn for \textsc{BiLSTM+Con} and \textsc{BiLSTM+Att}.
It is because the interactions between context and user history are effective yet complex, requiring well-designed merging mechanisms to exploit their joint effects.
% Among different variants of our proposed neural models, \textsc{BiLSTM+BiA} and \textsc{BiLSTM+Mem} outperform \textsc{BiLSTM} on both datasets by successfully modeling users' previous messages and their alignment with the topics of ongoing conversations. However, \textsc{BiLSTM+Con} and \textsc{BiLSTM+Att} perform even worse than \textsc{BiLSTM}, indicating such simple mechanisms are not able to capture useful information and correctly model it.
%The possible reason is that our model and \textsc{MemN2N} can be benefited from exploring the joint effects in conversation context and user history. \textsc{LSTM} and \textsc{BiLSTM}, however, only learns representations from conversation context.

$\bullet$~\textit{Bi-attention mechanism better aligns the users' interests and the conversation topics.} 
\textsc{BiLSTM+BiA} achieves the best AUC and F1 scores, significantly outperforming all other comparison models on both datasets. In particular, it beats \textsc{BiLSTM+Mem}, which also able to learn the interaction between user history and conversation content, indicating the effectiveness of bi-attention over memory networks in this task. 

Interestingly, comparing the results on the two datasets, we notice all models yield better recall and F1 on Twitter than Reddit. 
This is due to the fact that Reddit users are more likely to abandon conversations, reflected as the fewer number of entries in Table \ref{tab:stat}. Twitter users, on the other hand, tend to stay longer in the conversations, which encourages all models to predict the return of users. 

\input{figs/varying_context.tex}
% It might because our model, with the bidirectional attention learned from conversation context and user history, is able to capture interests of users from their chatting history and whether these interests can match the topics discussed in the conversation.
% Such representations can hence usefully indicate whether a user will come back or not.

%Last section has shown our superiority in predicting conversation re-entries. 

% \xingshan{I think the following two paragraphs should be placed in this section.}

\subsection{Predicting Re-entries with Varying Context and User History}\label{ssec:context-and-history}

Here we study the effects of varying conversation context and user history over re-entry prediction.

\paragraph{Results with Varying Context.}

We first discuss model performance given different amounts of conversation context by varying the number of user entries. 
Figure \ref{fig:diff_times} shows the F1 scores for predicting the first, second, and third re-entries. For predicting second or third re-entries, turns of current context until given user's second or third entry will be given. 
As can be seen, all models' performance monotonically increases when more context is observed. Our \textsc{BiLSTM+BiA} uniformly outperforms other methods in all setups. 
Interestingly, baseline \textsc{All-Yes} achieves the most performance gain when additional context is given. This implies that the more a user contributes to a conversation, the more likely they will come back. 
% Figure \ref{fig:diff_times} shows the F1 scores yielded by various models in predicting the first, second, and third re-entries, observed the context till the last entry of target user.
% As can be seen, all models perform better provided with more turns from target user, which is attributed to the richer information from target conversations to be exploited. 
% We also observe that our model achieves consistently better F1 scores given varying length of context, indicating the effectiveness of incorporating user chatting history for predicting re-entries. 
%Interestingly, baseline \textsc{All-Yes}'s performance increases quickly, achieving comparable F1 scores to our model when three turns are observed from the users. This indicates that users are more likely to continue engaging in a conversation is they have invested significant time in it.

% \xingshan{Another interesting observation is that performance of \textsc{All-Yes} increases quickly, 
% even achieving very close results to our model in predicting third re-entries. It means that, a user tends to continue the conversation if they has repeatedly participated in that conversation.}

\paragraph{Results with Varying User History.}

\input{figs/varying_history.tex}

%We have shown the impacts of conversation context in re-entry prediction. 
We further analyze how model performance differs when different amounts of messages are given in the user history. From Figure \ref{fig:diff_len}, we can see that it generally yields better F1 scores when more messages are available for the user history, suggesting the usefulness of chatting history to signal user re-entries. The performance on Reddit does not increase as fast as observed on Twitter, which may mainly because the context from Reddit conversations is often limited. 

% Here we present an analysis on how our model performs tackling target users with varying sparsity degree exhibited in their user history.
% Figure \ref{fig:diff_len} shows our F1 scores for target users having varying number of messages in their chatting history. 
% It is seen that, in general, better F1 scores are achieved when there are more messages in users' chatting history.
% We also notice that the Twitter curve is above the Reddit one, and exhibits to be more precipitous. The possible reason is that Twitter conversations have more turns in context (shown in Figure \ref{subfig:conv-context}), providing richer content to measure how conversation topics match user interests, especially when user interests can be better captured from more messages in user history.

\subsection{Further Discussion}\label{ssec:discussion}

% In this section, we carry out quantitative and qualitative analysis to further understand and interpret the prediction results by our proposed models. 
We further discuss our models with an ablation study and a case study to understand and interpret their prediction results.

\paragraph{Ablation Study.} 
%\xingshan{add two variants to compare.}
To examine the contribution of each component in our framework, we present an ablation study on first re-entry prediction task.
Table \ref{tab:ablation} shows the results of our best full model (\textsc{BiLSTM+BiA}) together with its variant without using turn-level auxiliary meta ${\bf a}_t$ (defined in Section \ref{ssec:model:io} to record user activity and replying relations in context), and that without structure modeling layer (to capture conversation discourse in context described in Section \ref{ssec:model:context}); also compared are variants without using user chatting history (described in Section \ref{ssec:model:user}).

\input{tables/ablation.tex}

Our full model yields the best F1 scores, showing the joint effects of context and user history can usefully indicate user re-entries.
We also see that auxiliary triples, though conveying simple meta data for context turns, are helpful in our task.
In addition, interestingly, conversation structure looks more effective in models leveraging user history, because they can learn deeper semantic relations between context turns and user chatting messages.

% Table \ref{tab:ablation} shows the results produced by our best full model (\textsc{BiLSTM+BiA}) and several variants. 
% First two are variants without user modeling layer (described in Section \ref{ssec:model:user}), while the first one use a long BiLSTM (instead of turn modeling plus structure modeling described in Section \ref{ssec:model:context}) to model the whole conversation, and the second one is exactly \textsc{BiLSTM} in Table~\ref{tab:main_res}.
% The other two variants are only without structure encoder or without auxiliary triple (which indicates turn replying information and user’s involvement pattern) in context modeling layer. 

% As can be seen, using two different BiLSTM layer to hierarchically model the turns and the whole conversation helps on improving precision, so as the overall F1 score. And removing user history, structure encoder or auxiliary triple certainly harms the performance, because of the failure on capturing user interests or information between turns.
% F1 score drops more on Twitter when structure encoder is removed, indicating its importance for Twitter conversations which are usually longer. Meanwhile, user history component is more critical for Reddit conversations, where more user messages can be accessed.

\paragraph{Case Study.} 
We further utilize a case study based on the sample conversations shown in Figure~\ref{fig:intro-example} to demonstrate what our model learns.
%how our model effectively make predictions. 
Table~\ref{tab:caseres} displays the outputs from different models on estimating how likely $\bf{U_1}$ will re-engage in conversation 1 ($\bf{C_1}$) and conversation 2 ($\bf{C_2}$), where $\bf{U_1}$ returns to the latter. 
All neural models successfully forecast that $\bf{U_1}$ is more likely to re-engage in $\bf{C_2}$, while only \textsc{BiLSTM+BiA} yields correct results (given threshold $0.5$). 

%To further understand why our model can effectively predict re-entries, we take the user and the conversations displayed in Figure~\ref{fig:intro-example} as an example and analyze what our model captures that help it make the right prediction.
% Recall that target user $\bf{U_1}$, once involved in both conversation 1 and 2, but only come back to conversation 2 later. 
% Table~\ref{tab:caseres} displays the outputs of different models estimating how likely $\bf{U_1}$ will re-engage conversation 1 ($c_1$) and 2 ($c_2$). 
% As we can see, only our model and \textsc{MemN2N} successfully forecast that $\bf{U_1}$ is more likely to re-engage $c_2$ than $c_1$, while our model gives higher confidence to such prediction.

\input{tables/sample_outputs.tex}

We further visualize the attention weights output by \textsc{BiLSTM+BiA}'s bi-attention mechanism with a heatmap in Figure \ref{fig:attention}. As can be seen, it assigns higher attention values to turns $\bf{T_2}$ and $\bf{T_3}$ in conversation $\bf{C_2}$, due to their topical similarity with user ${\bf U_1}$'s interests, i.e. movies, as inferred from their previous messages about \textit{Let Me In}. The attention weights then guide the final prediction for higher chance of re-entry to $\bf{C_2}$ rather than $\bf{C_1}$.

% To further analyze why our model can successfully predict $\bf{U_1}$'s re-entry to $c_1$ and $c_2$, we visualize the weights of our bi-attention in the heatmap of Figure \ref{fig:attention}. 
% As can be seen, our model distinguishes the learned representations for $c_1$ and $c_2$, where higher attention weights are assigned to turns T$_2$ and T$_3$ in $c_2$ because of the similar topics discussed in $c_2$ (movies \textit{Inception} and \textit{Memento}) and ${\bf U_1}$'s chatting history (movie \textit{Let Me In}). 
% %\xingshan{added some details}
% The high attention weights captured for $c_2$ further result in the relatively higher likelihood estimated for ${\bf U_1}$'s re-entry to $c_2$ rather than $c_1$. 

\input{figs/case_attention.tex}

\subsection{Comparing with Humans}\label{ssec:human}
We are also interested in how human performs for the first re-entry prediction task, in order to find out how challenging such a task is. To achieve this, we design a human evaluation. 
Concretely, from each dataset, we randomly sample $50$ users who have been involved in at least $4$ conversations, with both re-entry and non re-entry behaviors exhibited. 
Then for each user $u$, we construct paired samples based on randomly selected conversations $c_1$ and $c_2$, where $u$ re-engage in one but not the other. 
The rest of the conversations that $u$ participated in are collected as their user history. 
Then, we invite two humans who are fluent speakers of English, to predict which conversation user $u$ will re-engage, after reading the context up to user's first participation in the paired conversations $c_1$ and $c_2$. 
They are requested to make a second prediction after reading user's chatting history. 

\input{tables/human_eval.tex}

Humans' prediction performance is shown in Table~\ref{tab:he} along with \textsc{BiLSTM+BiA} model's output on the same data. 
%
As can be seen, humans can only give marginally better predictions than a random guess, i.e., 25 out of 50 pairs. Their performance improves after reading the user's previous posts, however, still falls behind our model's predictions. This indicates the ability of our model to learn from large-scaled data and align users' interests with conversation content. 
In addition, we notice that humans yield better performance on Reddit conversations than Twitter. It might be due to the fact that Reddit conversations are more focused, and it is easier for humans to identify the discussion points. While for Twitter discussions, the informal language usage further hinders humans' judgment.


% We have discussed the performance
% of various models on re-entry prediction. It is hence interesting to study how humans perform on this task. To this end, from each dataset, we randomly select $50$ users involved in at least $4$ conversations, exhibiting both re-entry and non re-entry behaviors in the conversations they participated in.
% For each user $u$, we randomly select two conversations $c_1$ and $c_2$, extracting their context turns with $u$ coming back later to only one of them.
% Then, we invite two annotators, both can speak English well, to forecast which conversation user $u$ will re-engage, after reading the context of $c_1$ and $c_2$. 
% Then, we ask them to read $u$'s chatting history and try again. 

% The predicted results from human and our model are shown in Table~\ref{tab:he}. 
% As can be seen, even humans work poorly on our task, though lightly better results are observed for the second try (with user history given). Such results indicate that re-entry prediction is challenging even for humans. 
% We also found that our model outperform humans on both datasets, perhaps owing to its ability to learn useful representations from large data. 
% In addition, we notice that human annotators exhibit better performance on Reddit than Twitter. It might because compared with Reddit, Twitter conversations concern wider range of topics and exhibit a more informal language style. Such nature somehow hinders the understanding of topics discussed in both conversation context and user history, and will further result in prediction errors.

% we print out and examine the internal representations of similarity computed by $f_{score}()$ of our model. Table~\ref{tab:caserep} displays related highest two similarity scores for two conversation. In conversation 1, the similarity scores are all negative, except for the highest one, showing that the user's chatting history matches not very well with the current conversation. But it is very different in conversation 2, where gives much higher score in similarity, and highest scores come from history H$_3$ and H$_4$ which discuss similar topic. And related turns are T$_2$ and T$_3$, indicating that these two turns are most relevant, which can be found reasonable, since final re-entry message (T$_5$) is actually related to T$_3$ (about film MEMENTO).



% \section{Experimental Results}
% In this section, we first discuss our main comparison results in Section~\ref{ssec:r1}. Then we display more results of different aspects in Section~\ref{ssec:r2}, including ablation study, results of different entry times before predicting, and results of different lengths of chatting history.
% We use a case in Section~\ref{ssec:r3} to provide further insights, following by a human evaluation result (Section~\ref{ssec:r4}).

% \subsection{Results for Main Experiment}
% \label{ssec:r1}
% Results for our main experiment are displayed in Table~\ref{tab:main_res}. We can find that our model performs best for both datasets in metrics of AUC and F1 Score, which proves that our model has overall nice results.

% For the baselines, \textsc{RANDOM} baseline perform unsurprisingly poorest. \textsc{NAIVE} baseline perform a lot better, but it is still poorer than other comparing methods because of the low precision. 
% %Although it has the highest recall due to the simple strategy of giving all samples positive labels.

% For the conventional method \textsc{CCCT}, we can find that it tends to produce higher precision, but much lower recall, which in result performs not so well in overall results.

% All the neural network based methods tend to produce higher recall, which can be seen as a sign of good methods, since we may not want to take the risk of missing any possible positive samples. The two RNN-based methods (\textsc{LSTM} and \textsc{BiLSTM}) perform very similar to \textsc{NAIVE} baseline, which means that they cannot guarantee the precision score while keeping their much higher recall. Both \textsc{MEMN2N} and Our Model has taken chatting history into consideration, and both produce higher precision, which implies that the chatting history plays a role in distinguishing re-entry behavior.

% Our model not only models the context structure in a conversation, but also gives a better connection using bidirectional attention mechanism between current conversation and user's chatting history. Therefore, our model can outperform all other methods.

% \subsection{Results for More Experiments}
% \label{ssec:r2}
% \paragraph{Ablation Study.} 
% Here we design an ablation study to further examine the related contributions of context structure and chatting history in our model, by eliminating either user history modeling layer (no history) or structure modeling layer (no hierarchical).
% %To further prove the effectiveness of our model, we design two variants of our model to do the experiments. The first variant is to show the performance without the effect of user's history, by eliminating the user's history modeling layer, and so that the bidirectional attention layer is also excluded. The second variant is to show the performance without the effect of hierarchical structure modeling, by eliminating the second BiLSTM in context modeling layer, and so that the context turn information $T_i$ is not counted. 
% We display the F1 Score results of these two kinds of variants as well as our model in Table~\ref{tab:ablation} for comparison. The results show that both variants perform worse that our full model. We can also find that the variant without history performs better in Twitter dataset, while in Reddit dataset it is contrary. This reflects the differences between these two platforms. In Twitter, users tend to discuss diverse topics, so the discussions from other conversations (chatting history) may be not very useful for prediction. But in Reddit, users discuss similar topics in a specific domain, so their previous words may be more important.



% \paragraph{Results with Different Degrees of Participation in Given Conversation.}
% Our main experiment is to predict whether given user will re-enter the given conversation, given their first entry to that conversation. Apparently it is the worthiest setting to be perform since the earlier we can make the prediction the better. However, we also want to know whether we can give more reliable prediction if we have more information about the current conversation. Therefore, we design an experiment to test the performance in another two settings: predicting re-entry behavior given the first two and three entries to the current conversation. The results in such settings, together with the results in main experiment for comparing, are displayed in Figure~\ref{fig:diff_times}.

% According to the results in Figure~\ref{fig:diff_times}, we can find that all models perform better, given more context in current conversation. One interesting observation is that the performance of \textsc{NAIVE} baseline increases quickly, and its results in given first 3 entries are actually very close to our model. It means that, in real situation, people tends to continue the conversation if they has repeatedly participated in that conversation. So the prediction of given more entries history seems meaningless.


% \paragraph{Results with Different Lengths of history.}
% Previous experiments have shown that user history is actually important for our task. Here we want to explore more about the effect of history. We design an experiment to test the performance of different users that have different lengths of history (i.e. total amount of posts in chatting history). An intuitive thinking is that, the more history information we have, the better we know about the current user, and so that we can provide better prediction for the user. Therefore, we divide the users in our test set into different groups, based on the lengths of their chatting history. The results are displayed in Figure~\ref{fig:diff_len}. The figure shows us that performance is indeed improved on the whole, as the length of history getting longer. The curve of Twitter gets some fluctuation, that's probably the dataset is relatively small, and number of samples with some lengths of history may not enough for reflecting general cases.



% \subsection{Case Study}
% \label{ssec:r3}
% In this section, we present a case study based on the example (Figure~\ref{fig:intro-example}) discussed in Section~\ref{sec:intro}. Recall that target user $\bf{U_1}$ whose history includes H$_1$ to H$_4$, has been involved in both conversation 1 and 2, but later only returns to conversation 2. Table~\ref{tab:caseres} displays the outputs of these two samples from our model and other comparisons. We can find that only our model gives a much higher score to conversation 2, which is exactly the user $\bf{U_1}$ returns. To further find out how our model can derive such results, we print out and examine the internal representations of similarity computed by $f_{score}()$ of our model. Table~ displays related highest two similarity scores for two conversation. In conversation 1, the similarity scores are all negative, except for the highest one, showing that the user's chatting history matches not very well with the current conversation. But it is very different in conversation 2, where gives much higher score in similarity, and highest scores come from history H$_3$ and H$_4$ which discuss similar topic. And related turns are T$_2$ and T$_3$, indicating that these two turns are most relevant, which can be found reasonable, since final re-entry message (T$_5$) is actually related to T$_3$ (about film MEMENTO).


% \subsection{Human Evaluation}
% \label{ssec:r4}
% Above experiments have shown the performance of different models and explain how our model can draw better performance. We can also see that although our model outperforms other models, all these models provide not good enough results (best f1 score $60.56$ for Twitter dataset and $44.63$ for Reddit dataset). In this section, we try to figure out whether it is such a difficult problem according to designing a human evaluation. We randomly choose 50 users that have participated in at least 4 conversations for two datasets, respectively. And each user has re-entered at least one of the conversations, not re-entered at least one of them. For each user, we select one sample with two conversations, and they only re-enter one of them. Rest conversations are for history. Then we hire two individuals who can read English posts fluently, to predict which one the given user will re-enter. We first let them predict without the information of history, and then predict again after reading the chatting history. 

% Table~\ref{tab:he} displays the results of such experiment. The results of our model derives from predicting the given user will re-enter the conversation with higher output (probability). From the result, we can find that: (1) it is a difficult task even for human to predict the re-entry behavior with so limited information, while our model can catch more information and predict better than human. (2) History information is useful for human predicting re-entry behavior. (3) Human gives better prediction in Reddit dataset, while our model predicts better in Twitter. This may be because topics discussed in Twitter are more diverse and hard for human to get a clear idea of user's preferences, but it would not be considered as a problem for our model.



==> ACL2019(final)/tables/ablation.tex <==
\begin{table}[th]
\begin{center}
\setlength{\tabcolsep}{1.3mm}
\fontsize{10}{11}\selectfont
\begin{tabular}{|l|lll|lll|}
\hline 
\multirow{2}{*}{\bf{Models}}&\multicolumn{3}{c|}{\bf Twitter}& \multicolumn{3}{c|}{\bf Reddit}\\
\cline{2-7}
&F1&Pre&Rec&F1&Pre&Rec\\
\hline
\underline{\bf W/O History} & & & & & & \\
W/O SML&58.8&42.6&\textbf{95.1}&39.6&25.2&\textbf{92.9}\\
With SML&59.4&45.9&85.0&43.1&31.4&69.5\\
\hline
\underline{\bf With History} & & & & & & \\
W/O SML&57.5&43.2&86.7&43.8&31.3&74.4\\
W/O Meta&60.4&46.6&86.1&44.3&31.3&75.8\\
Full model&\textbf{61.1}&\textbf{47.0}&87.7&\textbf{45.4}&\textbf{33.9}&68.9\\
\hline
\end{tabular} 
\end{center}
%\vspace{-2mm}
%\vskip -1em
\captionsetup{font=10pt}
\caption{Results of our variants.
SML: structure modeling layer. Meta: auxiliary triples ${\bf a}_t$.
Our full model \textsc{BiLSTM+BiA} obtains the best F1. 
%of different variants of our proposed model \textsc{BiLSTM+BiA}, by removing or replacing different components of proposed framework. 
%Our model (w/o user history): variant without user history modeling layer; Our model (w/o structure encoder): variant without structure encoder in context modeling layer.
}
%\vskip -1em
\label{tab:ablation}
\end{table}

==> ACL2019(final)/tables/comparison.tex <==
\begin{table*}
\begin{center}
%\setlength{\tabcolsep}{0.5mm}
\fontsize{11}{11}\selectfont
\begin{tabular}{|l|cccr|cccr|}
\hline
\multirow{2}{*}{\bf{Models}}&\multicolumn{4}{c|}{\bf Twitter}& \multicolumn{4}{c|}{\bf Reddit}\\
\cline{2-9}
&AUC&F1 Score&Precision&Recall&AUC&F1 Score&Precision&Recall\\
\hline
\underline{\bf Baselines} & & & & & & & & \\
\textsc{Random}&51.0&45.0&40.3&50.9&49.4&32.6&24.5&48.7 \\
\textsc{History}&50.1&46.4&42.2&51.4&50.7&35.2&26.9&50.9\\
\textsc{All-Yes}&50.0&54.9&37.9&\bf{100.0}&50.0&38.5&23.8&\bf{100.0}\\
\hline
\hline
\underline{\bf S.O.T.A} & & & & & & & & \\
\textsc{CCCT}&57.7&57.0&45.5&76.4&59.9&39.8&\bf{44.7}&36.0 \\
\hline
\hline
\underline{\bf W/O History} & & & & & & & & \\
\textsc{Avg-Embed}&60.4&59.0&43.5&91.8&63.7&42.4&31.0&67.2\\
\textsc{CNN}&58.8&59.1&43.2&93.5&64.0&42.8&31.1&68.5\\
\textsc{BiLSTM}&60.4&59.4&45.8&85.0&64.1&43.1&31.4&69.5\\
\hline
\hline
\underline{\bf With History} & & & & & & & & \\
\textsc{BiLSTM+Con}&51.0&58.0&40.9&\bf{100.0}&50.1&38.6&24.0&98.3\\
\textsc{BiLSTM+Att}&58.4&59.0&44.6&87.3&60.3&41.3&27.8&82.4\\
\textsc{BiLSTM+Mem}&61.3&59.9&45.7&87.5&65.5&43.7&31.8&69.9\\
\textsc{BiLSTM+BiA}&\bf{62.7}&\bf{61.1}&\bf{47.0}&87.7&\bf{67.1}&\bf{45.4}&33.9&68.9\\ 
\hline
\end{tabular}
\end{center}
%\vskip -1em
\captionsetup{font=10pt}
\caption{Results on first re-entry prediction. The best results in each column are in \textbf{bold}. Model \textsc{BiLSTM+BiA} yields significantly better AUC and F1 scores than all other comparisons ($p<0.05$, paired t-test). %\lu{xingshan, add $\ast$ for significant numbers by our models} \xingshan{the table seems too narrow for adding $\ast$}
%than all comparisons for AUC and F1 score at significance level of 0.05 in paired t-test.
}
%\vskip -1em
\label{tab:main_res}
\end{table*}



==> ACL2019(final)/tables/human_eval.tex <==
\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{4.0mm}
\fontsize{10}{11}\selectfont
\begin{tabular}{|l|c|c|}
\hline 
\bf{Predictor}&\bf{Twitter}&\bf{Reddit}\\
\hline
Human 1&26 ({\bf 29})&30 ({\bf 30})\\
Human 2&25 ({\bf 28})&28 ({\bf 29})\\
\textsc{BiLSTM+BiA}&35&33\\
\hline
\end{tabular} 
\end{center}
%\vskip -1em
\captionsetup{font=10pt}
\caption{
%\lu{i changed annotator to human, bold numbers}
Numbers of correct predictions made by humans, reading conversation context only and further seeing users' chatting history (boldfaced numbers), compared to the results of our best model in same setting. A random guess gives $25$ (out of $50$ pairs). 
%in parentheses). 
%in ``()'' refers to count of correct answers after humans read users' chatting history. 
%The number users  that is predicted correctly by different person and our model (The results in ``()'' are predicted after reading history information). The total amount is 50 for each dataset. 
}
%\vskip -1em
\label{tab:he}
\end{table}

==> ACL2019(final)/tables/statistics.tex <==
\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{1.0mm}
\fontsize{10}{11}\selectfont
\begin{tabular}{|l|r r|}
\hline 
%\bf{Properties}
&\bf{Twitter}&\bf{Reddit}\\
\hline
\# of users&10,122&13,134\\
\# of conversations&7,500&29,477\\
\# of re-entry instances&5,875&12,780\\
\# of non re-entry instances &8,677&39,988\\
\hline
%\# of turn&38,999&109,774\\
Avg. \# of convs per user&1.7&5.9\\
Avg. \# of msgs in user history &3.9&8.4\\
Avg. \# of entries per user per conv&2.0&1.3\\
Avg. \# of turns per conv&5.2&3.7\\
Avg. \# of users per conv&2.3&2.6\\

\hline
\end{tabular} 
\end{center}
%\vskip -1em
\captionsetup{font=10pt}
\caption{Statistics of two datasets.
%\lu{one digit after point it good}
}
%\vskip -1em
\label{tab:stat}
\end{table}
